Reachability in 3-VASS is Elementary

The reachability problem in 3-dimensional vector addition systems with states (3-VASS) is known to be PSpace-hard, and to belong to Tower. We significantly narrow down the complexity gap by proving the problem to be solvable in doubly-exponential space. The result follows from a new upper bound on the length of the shortest path: if there is a path between two configurations of a 3-VASS then there is also one of at most triply-exponential length. We show it by introducing a novel technique of approximating the reachability sets of 2-VASS by small semi-linear sets.

==> future-short.tex <==
% !TEX root = main.tex

\section{Future research}\label{sec:future}

We have shown that the shortest paths in binary \tvass is of at most triply-exponential length,
but we actually conjecture a doubly-exponential upper bound.
On the side of lower bound, it would be exciting to see an example of \tvass with doubly-exponential
shortest run, for instance by adapting the construction of 
\cite{DBLP:conf/concur/Czerwinski0LLM20}.
Also, a natural question is to ask if our approach is extendible to higher dimensions, e.g., to \parvass 4.
Another natural research direction is to seek for applications of \sandwich sets,
for instance to
\dvass extended with arbitrarily many $\Z$-counters.

